PrepNet: A Convolutional Auto-Encoder to Homogenize CT Scans for Cross-Dataset Medical Image Analysis

With the spread of COVID-19 over the world, the need arose for fast and precise automatic triage mechanisms to decelerate the spread of the disease by reducing human efforts e.g. for image-based diagnosis. Although the literature has shown promising efforts in this direction, reported results do not consider the variability of CT scans acquired under varying circumstances, thus rendering resulting models unfit for use on data acquired using e.g. different scanner technologies. While COVID-19 diagnosis can now be done efficiently using PCR tests, this use case exemplifies the need for a methodology to overcome data variability issues in order to make medical image analysis models more widely applicable. In this paper, we explicitly address the variability issue using the example of COVID-19 diagnosis and propose a novel generative approach that aims at erasing the differences induced by e.g. the imaging technology while simultaneously introducing minimal changes to the CT scans through leveraging the idea of deep auto-encoders. The proposed prepossessing architecture (PrepNet) (i) is jointly trained on multiple CT scan datasets and (ii) is capable of extracting improved discriminative features for improved diagnosis. Experimental results on three public datasets (SARS-COVID-2, UCSD COVID-CT, MosMed) show that our model improves cross-dataset generalization by up to $11.84$ percentage points despite a minor drop in within dataset performance.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> figures/figure_misclassification.tex <==
\centering
\begin{tabular}{l | c c  | c c}
    \toprule
    Preprocessing & \multicolumn{2}{c|}{Auto-encoder} & \multicolumn{2}{c}{\emph{PrepNet}} \\
    Dataset & SARS-COV-2 &  UCSD COVID-CT  & SARS-COV-2 &  UCSD COVID-CT \\
    \toprule
    Positive & 
    \includegraphics[width=3cm]{images/misclass/dataset0/ae_positive.png} &
    \includegraphics[width=3cm]{images/misclass/dataset1/ae_positive.png} &
    \includegraphics[width=3cm]{images/misclass/dataset0/prep_positive.png} &
    \includegraphics[width=3cm]{images/misclass/dataset1/prep_positive.png} \\
    \toprule
    Negative & 
    \includegraphics[width=3cm]{images/misclass/dataset0/ae_negative.png} &
    \includegraphics[width=3cm]{images/misclass/dataset1/ae_negative.png} &
    \includegraphics[width=3cm]{images/misclass/dataset0/prep_negative.png} &
    \includegraphics[width=3cm]{images/misclass/dataset1/prep_negative.png} \\
    \toprule     
\end{tabular}



==> figures/figure_preprocessing.tex <==
\centering
\begin{tabular}{l | c | c c c c c}
\toprule
Dataset & COVID & Original & Histogram equalization & Normalization & Auto-encoder & \emph{PrepNet} \\
\toprule
% SARS-COV-2 & Negative &
% \includegraphics[width=3.5cm]{images/dataset_0/negative/image_1.png} &
% \includegraphics[width=3.5cm]{images/dataset_0/negative/image_2.png} &
% \includegraphics[width=3.5cm]{images/dataset_0/negative/image_3.png} &
% \includegraphics[width=3.5cm]{images/dataset_0/negative/image_4.png} &
% \includegraphics[width=3.5cm]{images/dataset_0/negative/image_5.png}\\
% \midrule
SARS-COV-2 & Positive &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_2.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_3.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_4.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_5.png}\\
\toprule
UCSD COVID-CT & Negative &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_2.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_3.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_4.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_5.png}\\
% \midrule
% UCSD COVID-CT & Positive &
% \includegraphics[width=3.5cm]{images/dataset_1/positive/image_1.png} &
% \includegraphics[width=3.5cm]{images/dataset_1/positive/image_2.png} &
% \includegraphics[width=3.5cm]{images/dataset_1/positive/image_3.png} &
% \includegraphics[width=3.5cm]{images/dataset_1/positive/image_4.png} &
% \includegraphics[width=3.5cm]{images/dataset_1/positive/image_5.png}\\
\toprule     
\end{tabular}

==> figures/figure_presentation.tex <==
\centering
\begin{tabular}{l | c c}
\toprule
Dataset & Negative & Positive \\
\toprule
SARS-COV-2 &
\includegraphics[width=3.5cm]{images/dataset_0/negative/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_1.png} \\
\toprule
UCSD COVID-CT & 
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_1/positive/image_1.png} \\
\toprule     
\end{tabular}

==> figures/figure_visualization.tex <==
\centering
\begin{tabular}{l | c | c c c c c}
\toprule
Test Dataset
Training Dataset & Image (positive) & Original & Histogram equalization & Normalization & Auto-encoder & PrepNet \\
\toprule
SARS-COV-2 & Negative &
\includegraphics[width=3.5cm]{images/dataset_0/negative/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_0/negative/image_2.png} &
\includegraphics[width=3.5cm]{images/dataset_0/negative/image_3.png} &
\includegraphics[width=3.5cm]{images/dataset_0/negative/image_4.png} &
\includegraphics[width=3.5cm]{images/dataset_0/negative/image_5.png}\\
\midrule
SARS-COV-2 & Positive &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_2.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_3.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_4.png} &
\includegraphics[width=3.5cm]{images/dataset_0/positive/image_5.png}\\
\toprule
UCSD COVID-CT & Negative &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_2.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_3.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_4.png} &
\includegraphics[width=3.5cm]{images/dataset_1/negative/image_5.png}\\
\midrule
UCSD COVID-CT & Positive &
\includegraphics[width=3.5cm]{images/dataset_1/positive/image_1.png} &
\includegraphics[width=3.5cm]{images/dataset_1/positive/image_2.png} &
\includegraphics[width=3.5cm]{images/dataset_1/positive/image_3.png} &
\includegraphics[width=3.5cm]{images/dataset_1/positive/image_4.png} &
\includegraphics[width=3.5cm]{images/dataset_1/positive/image_5.png}\\
\toprule     
\end{tabular}

==> tables/dataset_backup.tex <==
\begin{table*}[htb]
    \begin{center}
    \caption{List of the used datasets}
    \label{tab:adatasets}
    \resizebox{0.98\textwidth}{!}{  
        \begin{tabular}{l|cccccccc}
            \toprule
            Name  & Task & Source & Patients  &  Format \cite{larobina2014medical} & Type & Size & Country \\ 
            \midrule
            %CT machine learning dataset \cite{maguolo2020critic}     & Classification & multiple & $>$20 & NIftI   & 3D & Various & Global & \url{https://github.com/ieee8023/covid-chestxray-dataset} \\
            %Lung infection segmentation dataset \cite{ma2020towards} & Both & multiple & $>$20 & NIftI & 3D & Various & Global & \url{https://zenodo.org/record/3757476#.Xpz8OcgzZPY} \\
            %SARS-COV-2 Ct-Scan Dataset \cite{soares2020sars} & Classification & single & 120 & png & Slice & Various& Brazil & \url{https://www.kaggle.com/plameneduardo/sarscov2-ctscan-dataset} \\
            SARS-COV-2 Ct-Scan Dataset2 \cite{DVN/SZDUQX_2020} & Classification & single &  210 & png & Slice & Various & Brazil  \\
            UCSD COVID-CT database \cite{zhao2020covid}              & Classification & multiple & $>$216 & png/jpg & Slice & Various & China \\
            %MosMed COVID-19 Chest CT database                        & Both & multiple & 1110  & NIftI & 3D & (512,512) & Russia & \url{https://mosmed.ai/datasets/covid19_1110} \\
            %COVID-19 CT segmentation dataset                         & Segmentation & single & $>$40 & NIftI  & Slice & (512,512) & Italy  & \url{http://medicalsegmentation.com/covid19/}  \\
            \toprule
        \end{tabular}
    }
    \end{center}
\end{table*}
%\url{https://gitee.com/junma11/COVID-19-CT-Seg-Benchmark}
%& \url{https://dataverse.harvard.edu/dataset.xhtml?persistentId=doi:10.7910/DVN/SZDUQX}
%& \url{https://github.com/UCSD-AI4H/COVID-CT}

==> tables/hyperparamters.tex <==
\begin{tabular}{l|cccc}
\toprule
Model &  Batch size & Learning rate & Weight decay & Dropout  \\     
\midrule
\midrule
& \multicolumn{4}{c}{Original} \\
\midrule
Classifier A &  4 & 1.2105e-06 & 2.7456e-05 & 0.7 \\
Classifier B & 64 & 6.4351e-05 & 5.2989e-07 & 0.5  \\  
\midrule
\midrule
& \multicolumn{4}{c}{Autoencoder} \\
\midrule
Autoencoder  & 4 & 4.5196e-6 & - & - \\
Classifier A & 32 & 1.0947e-6 & 3.6337e-6 & 0.4 \\
Classifier B & 64 & 1.5916e-6 & 5.8231e-4 & 0.2  \\   
\midrule
\midrule
& \multicolumn{4}{c}{PrePnet} \\
\midrule
PrePnet      &  4 & 2.7177e-4 & 2.7177e-4 & 0.7  \\
Classifier A &  4 & 3.5532e-7 & 3.0100e-7 & 0.7 \\
Classifier B & 32 & 4.6515e-7 & 6.7779e-7 & 0.2 \\  
\midrule
\toprule
\end{tabular}

==> tables/table_covid.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|cccc|cccc|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{4}{c|}{SARS-COV-2} & \multicolumn{4}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset   \\ 
        Dataset portion  & Train & Validation & Test & Average & Train & Validation & Test & Average & Average & Average \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{10}{c}{Original} \\
        \midrule
        SARS-COV-2      & $0.9533$ & $\boldsymbol{0.9366}$ & $0.8303$ &        - & $0.4193$ & $0.3310$ & $0.4813$ & $0.4105$ & $\boldsymbol{0.7890}$    & $0.4503$ \\
        UCSD COVID-CT   & $0.5084$ & $0.4848$ & $0.4770$ & $0.4901$ & $\boldsymbol{0.8101}$ & $0.6183$ & $\boldsymbol{0.7478}$ &        - & (Baseline)  & (Baseline) \\         
        \midrule
        \midrule
        & \multicolumn{10}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2      & $0.9414$ & $0.8980$ & $0.6574$ &        - & $\boldsymbol{0.5159}$ & $0.5006$ & $\boldsymbol{0.5041}$ & $\boldsymbol{0.5069}$ & $0.7026$     & $\boldsymbol{0.5209}$ \\
        UCSD COVID-CT   & $\boldsymbol{0.5456}$ & $\boldsymbol{0.5173}$ & $\boldsymbol{0.5421}$ & $\boldsymbol{0.5350}$ & $0.7934$ & $\boldsymbol{0.7186}$ & $0.7337$ &        - & ($-8.64\%$)  & ($\boldsymbol{+7.06\%}$)\\         
        \midrule
        \midrule
        & \multicolumn{10}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2      & $\boldsymbol{0.9786}$ & $0.8157$ & $\boldsymbol{0.8352}$ &        - & $0.5054$ & $\boldsymbol{0.5094}$ & $0.4835$ & $0.4994$  & $0.7721$    & $0.5002$ \\
        UCSD COVID-CT   & $0.5010$ & $0.4173$ & $0.5037$ & $0.4740$ & $0.7279$ & $0.6390$ & $0.7090$ &         - & ($\boldsymbol{-1.69\%}$) & ($+4.99\%$) \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_detailed.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|ccc|ccc|ccc}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{9}{c}{SARS-COV-2} \\ 
        Dataset portion  & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test} \\
        Metrics  & Recall & Precision & F1-score & Recall & Precision & F1-score & Recall & Precision & F1-score  \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{9}{c}{Original} \\
        \midrule
        SARS-COV-2 & $0.9802$ & $0.9744$ & $0.9773$ & $0.9785$ & $0.9636$ & $0.9710$ & $0.9938$ & $0.8947$ & $0.9417$ \\
        UCSD COVID-CT & $0.4193$ & $0.1107$ & $0.5385$ & $0.1837$ & $0.3310$ & $0.0831$ & $0.3600$ & $0.1350$ & $0.4813$ \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2 & $0.9980$ & $0.9613$ & $0.9793$ & $0.9538$ & $0.9451$ & $0.9495$ & $0.9815$ & $0.8076$ & $0.8861$ \\
        UCSD COVID-CT & $0.5456$ & $0.4107$ & $0.7866$ & $0.5396$ & $0.5173$ & $0.3415$ & $0.7603$ & $0.4713$ & $0.5421$  \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2 & $0.9703$ & $0.9953$ & $0.9826$ & $0.8769$ & $0.9105$ & $0.8934$ & $0.8985$ & $0.9182$ & $0.9082$ \\
        UCSD COVID-CT & $0.5010$ & $0.7581$ & $0.7419$ & $0.7499$ & $0.4173$ & $0.5538$ & $0.6870$ & $0.6133$ & $0.5037$ \\     \toprule    
        \toprule
                Test dataset $\rightarrow$ & \multicolumn{9}{c}{UCSD COVID-CT} \\ 
        Dataset portion  & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test} \\
        Metrics  & Recall & Precision & F1-score & Recall & Precision & F1-score & Recall & Precision & F1-score  \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{9}{c}{Original} \\
        \midrule
        SARS-COV-2 & $0.9053$ & $0.4538$ & $0.6046$ & $0.8644$ & $0.5000$ & $0.6335$ & $0.8866$ & $0.4699$ & $0.6143$  \\
        UCSD COVID-CT & $0.8101$ & $0.6632$ & $0.9265$ & $0.7730$ & $0.6183$ & $0.2542$ & $0.9375$ & $0.4000$ & $0.7478$ \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2 & $0.9632$ & $0.4575$ & $0.6203$ & $0.9661$ & $0.5089$ & $0.6667$ & $0.9794$ & $0.4847$ & $0.6485$ \\
        UCSD COVID-CT & $0.7934$ & $0.6211$ & $0.9365$ & $0.7468$ & $0.7186$ & $0.5424$ & $0.8421$ & $0.6598$ & $0.7337$  \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2 & $0.9421$ & $0.4520$ & $0.6109$ & $0.9661$ & $0.5135$ & $0.6706$ & $0.9381$ & $0.4740$ & $0.6298$ \\
        UCSD COVID-CT & $0.7279$ & $0.5632$ & $0.8106$ & $0.6646$ & $0.6390$ & $0.5763$ & $0.6667$ & $0.6182$ & $0.7090$ \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_effinet.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|cccc|cccc|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{4}{c|}{SARS-COV-2} & \multicolumn{4}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset   \\ 
        Dataset portion  & Train & Validation & Test & Average & Train & Validation & Test & Average & Average & Average \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{10}{c}{Original} \\
        \midrule
        SARS-COV-2    & $0.9660$ & $0.9469$ & $0.7452$ & - & $0.5844$ & $0.5665$ & $0.4696$ & $0.5402$ & $0.7161$ & $0.4713$  \\
        UCSD COVID-CT & $0.4871$ & $0.3931$ & $0.3272$ & $0.4025$ & $0.7401$ & $0.7264$ & $0.6870$ & - & (Baseline) & (Baseline) \\         
        \midrule
        \midrule
        & \multicolumn{10}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2    &  $0.9200$ & $0.8897$ & $0.7449$ & - & $0.4998$ & $0.4833$ & $0.5075$ & $0.4969$ & $0.7615$ & $0.4084$ \\
        UCSD COVID-CT &$0.3940$ & $0.3133$ & $0.2523$ & $0.3199$ & $0.9547$ & $0.8363$ & $0.7781$ & - & ($+4.54$\%) & ($-6.29$\%)\\         
        \midrule
        \midrule
        & \multicolumn{10}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2    & $0.9239$ & $0.7218$ & $0.8264$ & - & $0.4931$ & $0.4846$ & $0.4985$ & $0.4921$ & $0.6776$ & $0.5115$ \\
        UCSD COVID-CT & $0.5657$ & $0.5202$ & $0.5071$ & $0.5310$ & $0.5248$ & $0.5263$ & $0.5288$ & - & ($-3.85$\%) & ($+4.02$\%) \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_effinet_detailed.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|ccc|ccc|ccc}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{9}{c}{SARS-COV-2} \\ 
        Dataset portion  & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test} \\
        Metrics  & Recall & Precision & F1-score & Recall & Precision & F1-score & Recall & Precision & F1-score  \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{9}{c}{Original} \\
        \midrule
        SARS-COV-2    & $0.9848$ & $0.9816$ & $0.9832$ & $0.9815$ & $0.9696$ & $0.9755$ & $0.9815$ & $0.8507$ & $0.9114$ \\
        UCSD COVID-CT & $0.4871$ & $0.3843$ & $0.7288$ & $0.5032$ & $0.3931$ & $0.3477$ & $0.6384$ & $0.4502$ & $0.3272$ \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2    & $0.9743$ & $0.9542$ & $0.9641$ & $0.9723$ & $0.9349$ & $0.9532$ & $0.9723$ & $0.8518$ & $0.9080$ \\
        UCSD COVID-CT & $0.3940$ & $0.4779$ & $0.6651$ & $0.5562$ & $0.3133$ & $0.3108$ & $0.5642$ & $0.4008$ & $0.2523$  \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2    & $0.9499$ & $0.9639$ & $0.9568$ & $0.9262$ & $0.8455$ & $0.8840$ & $0.8985$ & $0.9125$ & $0.9054$ \\
        UCSD COVID-CT & $0.4931$ & $0.9862$ & $0.7388$ & $0.8447$ & $0.4846$ & $0.9692$ & $0.7343$ & $0.8355$ & $0.4985$ \\     \toprule    
        \toprule
                Test dataset $\rightarrow$ & \multicolumn{9}{c}{UCSD COVID-CT} \\ 
        Dataset portion  & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test} \\
        Metrics  & Recall & Precision & F1-score & Recall & Precision & F1-score & Recall & Precision & F1-score  \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{9}{c}{Original} \\
        \midrule
        SARS-COV-2    & $0.7053$ & $0.5174$ & $0.5969$ & $0.7119$ & $0.5600$ & $0.6269$ & $0.3814$ & $0.4458$ & $0.4111$ \\
        UCSD COVID-CT & $0.7401$ & $0.5789$ & $0.8271$ & $0.6811$ & $0.7264$ & $0.5932$ & $0.8140$ & $0.6863$ & $0.6870$ \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2    & $0.9053$ & $0.4491$ & $0.6003$ & $0.9492$ & $0.5000$ & $0.6550$ & $0.9381$ & $0.4866$ & $0.6408$ \\
        UCSD COVID-CT & $0.9547$ & $0.9737$ & $0.9250$ & $0.9487$ & $0.8363$ & $0.8305$ & $0.8448$ & $0.8376$ & $0.7781$  \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2    & $0.8053$ & $0.4935$ & $0.6120$ & $0.8475$ & $0.5208$ & $0.6452$ & $0.7835$ & $0.4872$ & $0.6008$ \\
        UCSD COVID-CT & $0.5248$ & $0.9895$ & $0.4619$ & $0.6298$ & $0.5263$ & $1.0000$ & $0.5221$ & $0.6860$ & $0.5288$ \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_old.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|cccc|cccc|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{4}{c|}{SARS-COV-2} & \multicolumn{4}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset   \\ 
        Dataset portion  & Train & Validation & Test & Average & Train & Validation & Test & Average & Average & Average \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{8}{c}{Original} \\
        \midrule
        SARS-COV-2 & $0.9658$ & $0.9586$ & \textbf{0.9074} & - & \textbf{0.4308} & $0.3894$ & $0.4914$ & $0.4372$ & $\boldsymbol{0.8590}$ & $0.3402$ \\
        UCSD COVID-CT & $0.2733$ & $0.1887$ & $0.2684$ & $0.2433$ & \textbf{0.8539} & $0.8039$ & \textbf{0.8106} & - & (Baseline) & (Baseline) \\         
        \midrule
        \midrule
        & \multicolumn{8}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2 & $0.9723$ & \textbf{0.9452} & $0.8420$ & - & $0.4252$ & $0.3797$ & \textbf{0.5089} & 0.4379 & 0.8085 & $0.4371$ \\
        UCSD COVID-CT & $0.4884$ & $0.3768$ & $0.4438$ & $0.4363$ & $0.8556$ & \textbf{0.8726} & $0.7703$ & - & ($-5.05$\%) & ($+9.68$\%) \\         
        \midrule
        \midrule
        & \multicolumn{8}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2 & \textbf{0.9775} & $0.8596$ & $0.8649$ & - & $0.4061$ & \textbf{0.3984} & $0.4041$ & $0.4028$ & $0.8099$ & $\boldsymbol{0.4959}$ \\
        UCSD COVID-CT & \textbf{0.6219} & \textbf{0.4734} & \textbf{0.6720} & $0.5891$ & $0.7802$ & $0.6095$ & $0.7550$ & - & ($-4.91$\%) & ($+15.57$\%) \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_resnet.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|cccc|cccc|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{4}{c|}{SARS-COV-2} & \multicolumn{4}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset   \\ 
        Dataset portion  & Train & Validation & Test & Average & Train & Validation & Test & Average & Average & Average \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{10}{c}{Original} \\
        \midrule
        SARS-COV-2    & $0.9971$ & $0.9642$ & $0.8444$ & - & $0.5343$ & $0.5112$ & $0.4975$ & $0.5143$ & $0.7520$ & $0.4153$  \\
        UCSD COVID-CT & $0.4015$ & $0.3052$ & $0.2426$ & $0.3164$ &  $0.7767$ & $0.7304$ & $0.6596$  & - & (Baseline) & (Baseline) \\         
        \midrule
        \midrule
        & \multicolumn{10}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2    & $0.9699$ & $0.9355$ & $0.9070$ & - & $0.5708$ & $0.4630$ & $0.4298$ & $0.4879$ & $0.8257$ & $0.4237$  \\
        UCSD COVID-CT & $0.3938$ & $0.3832$ & $0.3015$ & $0.3595$ & $0.9064$ & $0.7001$ & $0.7444$  & - & ($+7.37$\%) & ($+0.84$\%) \\         
        \midrule
        \midrule
        & \multicolumn{10}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2    & $0.9765$ & $0.8347$ & $0.8121$ & - & $0.5298$ & $0.5296$ & $0.4167$ & $0.4920$ & $0.7725$ & $0.4980$ \\
        UCSD COVID-CT & $0.5648$ & $0.4377$ & $0.5097$ & $0.5041$ & $0.9713$ & $0.6738$ & $0.7330$ & - & ($+2.05$\%) & ($+8.27$\%) \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_resnet_detailed.tex <==
\resizebox{1.0\textwidth}{!}{  
    \begin{tabular}{l|ccc|ccc|ccc}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{9}{c}{SARS-COV-2} \\ 
        Dataset portion  & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test} \\
        Metrics  & Recall & Precision & F1-score & Recall & Precision & F1-score & Recall & Precision & F1-score  \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{9}{c}{Original} \\
        \midrule
        SARS-COV-2    & $0.9980$ & $0.9987$ & $0.9984$ & $0.9723$ & $0.9844$ & $0.9783$ & $0.9169$ & $0.9198$ & $0.9183$ \\
        UCSD COVID-CT & $0.4015$ & $0.4608$ & $0.6676$ & $0.5452$ & $0.3052$ & $0.3385$ & $0.5699$ & $0.4247$ & $0.2426$ \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2    & $0.9492$ & $0.9965$ & $0.9723$ & $0.9323$ & $0.9774$ & $0.9543$ & $0.9631$ & $0.9485$ & $0.9557$ \\
        UCSD COVID-CT & $0.3938$ & $0.2281$ & $0.5976$ & $0.3302$ & $0.3832$ & $0.3015$ & $0.6164$ & $0.4050$ & $0.3015$  \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2    & $0.9624$ & $0.9966$ & $0.9792$ & $0.8185$ & $0.9399$ & $0.8750$ & $0.7908$ & $0.9312$ & $0.8552$  \\
        UCSD COVID-CT & $0.5648$ & $0.6684$ & $0.7806$ & $0.7202$ & $0.4377$ & $0.6123$ & $0.7032$ & $0.6546$ & $0.5097$ \\     \toprule    
        \toprule
                Test dataset $\rightarrow$ & \multicolumn{9}{c}{UCSD COVID-CT} \\ 
        Dataset portion  & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Validation} & \multicolumn{3}{c}{Test} \\
        Metrics  & Recall & Precision & F1-score & Recall & Precision & F1-score & Recall & Precision & F1-score  \\
        \midrule
        \midrule
        Training dataset $\downarrow$ & \multicolumn{9}{c}{Original} \\
        \midrule
        SARS-COV-2    & $0.8368$ & $0.4704$ & $0.6023$ & $0.8644$ & $0.5152$ & $0.6456$ & $0.7835$ & $0.4810$ & $0.5961$ \\
        UCSD COVID-CT & $0.7767$ & $0.9526$ & $0.6606$ & $0.7802$ & $0.7304$ & $0.8644$ & $0.6892$ & $0.7669$ & $0.6596$ \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{Auto-Encoder} \\
        \midrule
        SARS-COV-2    & $0.7211$ & $0.5037$ & $0.5931$ & $0.6102$ & $0.4800$ & $0.5373$ & $0.4845$ & $0.4196$ & $0.4498$ \\
        UCSD COVID-CT & $0.9064$ & $0.9158$ & $0.8788$ & $0.8969$ & $0.7001$ & $0.5932$ & $0.7609$ & $0.6667$ & $0.7444$  \\         
        \midrule
        \midrule
        & \multicolumn{9}{c}{\emph{PrepNet}} \\
        \midrule
        SARS-COV-2    & $0.6947$ & $0.4714$ & $0.5617$ & $0.8136$ & $0.5275$ & $0.6400$ & $0.5258$ & $0.4146$ & $0.4636$ \\
        UCSD COVID-CT & $0.9713$ & $0.9684$ & $0.9684$ & $0.9684$ & $0.6738$ & $0.5932$ & $0.7143$ & $0.6481$ & $0.7330$ \\         
        \toprule
    \end{tabular}
}

==> tables/table_covid_vgg19.tex <==
\begin{table*}
\centering
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|c|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{5}{c|}{SARS-COV-2} & \multicolumn{5}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset & Pre-trained  \\ 
        Dataset portion  & Test & Avg & Sens     & Spec     & AUC      & Test    & Avg  & Sens      & Spec     & AUC    & Average & Average & encoder\\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{Original} - grayscaling} \\
        \midrule
        SARS-COV-2***      &  &        - &  &  &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT***   &  &  &  &  &  &  &        - &  &  &  & (baseline) & (baseline) & \\ 
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{AutoEncoder} - grayscaling} \\
        \midrule
        SARS-COV-2 ***     & &        - & &  &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT   &  &  &  &  &  &  &        - &  &  &  & ($+\%$) & ($-\%$) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{PrepNet} - grayscaling} \\
        \midrule
        SARS-COV-2      &  &        - &  &  &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT   &  &  &  &  &  &  &        - &  &  &  & ($+\%$) & ($+\%$) & \\
        \toprule
    \end{tabular}}
    \caption{Test performance of different pre-processing schemes.}
\end{table*}

==> tables2/backbones.tex <==
\begin{table*}
\centering
\label{tab:prepnet_backbones}
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|c|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{5}{c|}{SARS-COV-2} & \multicolumn{5}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset & Pre-trained  \\ 
        Dataset portion  & Test & Avg & Sens     & Spec     & AUC      & Test    & Avg  & Sens      & Spec     & AUC    & Average & Average & encoder\\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{VGG19} - grayscaling} \\
        \midrule
         SARS-COV-2      & $0.9136$ &        - & $0.9415$ & $0.8407$ & $0.9491$ & $0.4633$ & $0.5384$ & $0.6907$ & $0.2524$ & $0.4867$ & $0.8393$ & $0.5880$ & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.7242$ & $0.6377$ & $0.8769$ & $0.2920$ & $0.5615$ & $0.7650$ &        - & $0.8350$ & $0.6990$ & $0.8665$ & (baseline) & (baseline) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{ResNet18} - grayscaling} \\
        \midrule
         SARS-COV-2      & $0.8742$ &        - & $0.9600$ & $0.6283$ & $0.9354$ & $0.4504$ & $0.4806$ & $0.8865$ & $0.0384$ & $0.4058$ & $0.8468$ & $0.4666$ & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.3909$ & $0.4486$ & $0.4461$ & $0.2304$ & $0.2714$ & $0.8193$ &        - & $0.8659$ & $0.7788$ & $0.9035$ & ($+0.75\%$) & ($-12.14\%$) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{ResNet50} - grayscaling} \\
        \midrule
        SARS-COV-2      & 0.9412 &        - & 0.8053 & 0.8769 & 0.8568 & 0.4930 & 0.5478 & 0.0874 & 0.8350 & 0.4533 & 9 & 10 & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & 0.2740 & 0.3526 &  0.4159 & 0.1784 & 0.2432 & 0.8792 &        - & 0.9029 & 0.6495 & 0.7800 & ($+\%$) & ($+\%$) & \\
                \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{Inception} - grayscaling} \\
        \midrule
        SARS-COV-2      &  &        - &  &  &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT   &  &  &  &  &  &  &        - &  &  &  & ($+\%$) & ($+\%$) & \\
                \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{EfficientNet-B0} - grayscaling} \\
        \midrule
        SARS-COV-2      &  &        - &  &  &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT   &  &  &  &  &  &  &        - &  &  &  & ($+\%$) & ($+\%$) & \\
        \toprule
    \end{tabular}}
    \caption{\emph{PrepNet} gray-scale with different backbones.}
\end{table*}

==> tables2/backbones2_avg.tex <==
\begin{table*}
\centering
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|c|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{5}{c|}{SARS-COV-2} & \multicolumn{5}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset & Pre-trained  \\ 
        Dataset portion  & Test & Avg & Sens     & Spec     & AUC      & Test    & Avg  & Sens      & Spec     & AUC    & Average & Average & encoder\\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{VGG19} - grayscaling} \\
        \midrule
         SARS-COV-2      & $0.9007$ &        - & $0.9353$ & $0.7982$ & $0.8668$ & $0.5157$ & $0.5298$ & $0.9175$ & $0.1067$ & $0.5121$ & $0.8404$ & $0.5343$ & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.5545$ & $0.5388$ & $0.6446$ & $0.1858$ & $0.4852$ & $0.7800$ &        - & $0.8556$ & $0.7087$ & $0.7822$ & ($-1.83\%$) & ($+11.84\%$) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{ResNet18} - grayscaling} \\
        \midrule
          SARS-COV-2       &  $0.7462$  & - & $0.7046$ & $0.8584$ & $0.7815$ & $0.4728$ & - & $0.8144$ & $0.1538$ & $0.4841$ & & & \multirow{2}*{Yes}\\
        UCSD COVID-CT & $0.5152$ & - & $0.6246$ & $0.1947$ & $0.4096$ & $0.7228$ & - & $0.8351$ & $0.6154$ & $0.7252$  & (baseline) & (baseline) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{ResNet50} - grayscaling} \\
        \midrule
         SARS-COV-2       & $0.6674$ & - & $0.7785$ & $0.3451$ & $0.5618$ &  $0.43069$ & - & $0.78351$ & $0.1058$ & $0.4446$ & & & \multirow{2}*{Yes}\\
        UCSD COVID-CT & $0.2083$ & - & $0.1908$ & $0.2478$ & $0.2193$ & $0.8168$ & - & $0.8557$ & $0.77885$ & $0.8172$ & (baseline) & (baseline) & \\
                \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{Inception} - grayscaling} \\
        \midrule
        SARS-COV-2      &  $0.8553$ & - & $0.9046$ & $0.7080$ & $0.8063$ & $0.4703$ & - & $0.9485$ & $0.02885$ & $0.4886$ & & & \multirow{2}*{Yes}\\
        UCSD COVID-CT & $0.3288$ & - & $0.36308$ & $0.2212$ & $0.2922$ & $0.8020$ & - & $0.8351$ & $0.7692$ & $0.8021$  & ($+\%$) & ($+\%$) & \\
                \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{EfficientNet-B0} - grayscaling} \\
        \midrule
        SARS-COV-2      & $0.8735$ & - & $0.8923$ & $0.8142$ & $0.8532$ & $0.5223$ & - & $0.5979$ & $0.4519$ & $0.5249$ & & & \multirow{2}*{Yes}\\
        UCSD COVID-CT & $0.4447$ & - & $0.5015$ & $0.2743$ & $0.3879$ & $0.7772$ & - & $0.8041$ &  $0.7500$ & $0.7771$ & ($+\%$) & ($+\%$) & \\
        \toprule
    \end{tabular}}
    \caption{\emph{PrepNet} gray-scale with different backbones.}
\end{table*}

==> tables2/mosmed_eval_avg.tex <==
\begin{table}
\centering
\resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l|ccccc|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{5}{c|}{MosMed} &   Pre-trained  \\ 
        Dataset portion  & Test & Avg & Sens     & Spec     & AUC & encoder\\
        \midrule
        \midrule
        & \multicolumn{5}{c}{\emph{COVID classifier} - grayscaling} \\
        \midrule
        SARS-COV-2      & $0.6066$ & $0.5942$ & $0.5246$ & $0.8771$ & $0.7009$ &    \multirow{4}*{Yes}\\
        & (baseline) & (baseline) & (baseline) & (baseline) & (baseline) & \\ 
        UCSD COVID-CT   & $0.2320$ & $0.2308$ & $0.0051$ & $1.000$ & $0.5025$ & \\
           & (baseline) & (baseline) & (baseline) & (baseline) & (baseline) & \\ 
        \midrule
        \midrule
        & \multicolumn{5}{c}{\emph{AutoEncoder} - grayscaling} \\
        \midrule
        SARS-COV-2      & $0.6693$ & $0.6712$ & $0.7142$ & $0.5175$ & $0.6159$ &   \multirow{4}*{Yes}\\
                        &  ($+6.27\%$) & ($+7.70\%$) & ($+18.96\%$) & ($-35.96\%$) & ($-8.50\%$) \\
        UCSD COVID-CT   & $0.2320$ & $0.2308$ & $0.0051$ & $1.000$ & $0.5025$ & \\
                        &  ($+0.00\%$) & ($+0.00\%$) & ($+0.00\%$) & ($+0.00\%$) & ($+0.00\%$) \\
        \midrule
        \midrule
        & \multicolumn{5}{c}{\emph{PrepNet} - grayscaling} \\
        \midrule
        SARS-COV-2      & $0.7073$ & $0.7066$ & $0.7558$ & $0.5438$ & $0.6498$ &  \multirow{4}*{Yes}\\
                        & ($+10.07\%$) & ($+11.24\%$) & ($+23.12\%$) & ($-33.33\%$) & ($-5.11\%$) \\
        UCSD COVID-CT   & $0.2520$ & $0.2431$ & $0.0181$ & $1.000$ & $0.5160$ \\
                        & ($+2.00\%$) & ($+1.23\%$) & ($+1.30\%$) & ($+0.00\%$) & ($+1.35\%$) \\
        \toprule
    \end{tabular}}
    \caption{\emph{PrepNet} gray-scale with different backbones.}
\end{table}

==> tables2/table_covid_vgg19_2.tex <==
\begin{table*}
\centering
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|c|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{5}{c|}{SARS-COV-2} & \multicolumn{5}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset & Pre-trained  \\ 
        Dataset portion  & BA & Avg & Sens     & Spec     & AUC      & BA    & Avg  & Sens      & Spec     & AUC    & Average & Average & encoder\\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{COVID classifier} - grayscaling} \\
        \midrule
        SARS-COV-2      &   &        - &   &   &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT & $0.6545$ & - & $0.7508$ & $0.3717$ & $0.5612$  & $0.6757$ & - & $0.7113$ & $0.6442$ & $0.6778$   &  (baseline) & (baseline)  \\ 
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{AutoEncoder} - grayscaling} \\
        \midrule
        SARS-COV-2      & &        - & &  &  &  &  &  &  &  &  &  & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.6288$ & - & $0.6831$ & $0.4690$ & $0.5761$ & $0.7079$ & - & $0.6289$ & $0.7788$ & $0.7039$ & ($+\%$) & ($-\%$) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{PrepNet} - grayscaling} \\
        \midrule
         SARS-COV-2      &  &        - &   &   &    &   &   &   &   &   &   &   & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.6470$ & - & $0.7015$ & $0.4867$ & $0.5941$ & $0.6782$ & - & $0.6082$ & $0.7404$ & $0.6743$  & ($+\%$) & ($+\%$) & \\
        \toprule
    \end{tabular}}
    \caption{Test performance of different pre-processing schemes.}
\end{table*}

==> tables2/table_covid_vgg19_avg.tex <==
\begin{table*}
\centering
\label{tab:covid_baselines_avg}
\resizebox{1.0\textwidth}{!}{
    \begin{tabular}{l|ccccc|ccccc|c|c|c}
        \toprule
        Test dataset $\rightarrow$ & \multicolumn{5}{c|}{SARS-COV-2} & \multicolumn{5}{c|}{UCSD COVID-CT} & Within Test & Cross-Dataset & Pre-trained  \\ 
        Dataset portion  & Test & Avg & Sens     & Spec     & AUC      & Test    & Avg  & Sens      & Spec     & AUC    & Average & Average & encoder\\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{COVID classifier} - grayscaling} \\
        \midrule
        SARS-COV-2      & $0.8924$ &        - & $0.9292$ & $0.7876$ & $0.8584$ & $0.4433$ & $0.4603$ & $0.7835$ & $0.1262$ & $0.4548$ & $0.8587$ & $0.4159$ & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.3295$ & $0.3715$ & $0.3476$ & $0.2743$ & $0.3110$ & $0.8250$ &        - & $0.7113$ & $0.9320$ & $0.8216$ & (baseline) & (baseline) & \\ 
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{AutoEncoder} - grayscaling} \\
        \midrule
        SARS-COV-2      & $0.8956$ &        - & $0.9907$ & $0.6460$ & $0.8183$ & $0.4983$ & $0.5034$ & $0.9175$ & $0.0970$ & $0.5073$ & $0.8555$ & $0.4836$ & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.49405$ & $0.4638$ & $0.6030$ & $0.3008$ & $0.4519$ & $0.8154$ &        - & $0.7216$ & $0.8846$ & $0.8031$ & ($-0.32\%$) & ($+6.77\%$) & \\
        \midrule
        \midrule
        & \multicolumn{13}{c}{\emph{PrepNet} - grayscaling} \\
        \midrule
         SARS-COV-2      & $0.9007$ &        - & $0.9353$ & $0.7982$ & $0.8668$ & $0.5157$ & $0.5298$ & $0.9175$ & $0.1067$ & $0.5121$ & $0.8404$ & $0.5343$ & \multirow{2}*{Yes}\\
        UCSD COVID-CT   & $0.5545$ & $0.5388$ & $0.6446$ & $0.1858$ & $0.4852$ & $0.7800$ &        - & $0.8556$ & $0.7087$ & $0.7822$ & ($-1.83\%$) & ($+11.84\%$) & \\
        \toprule
    \end{tabular}}
    \caption{Test performance of different pre-processing schemes.}
\end{table*}
